Mining Legal Arguments in U.S. Corporate Case Law

Legal argument mining supports passage classification, retrieval, and argument completion. This work introduces an expert-annotated dataset of 42 U.S. federal tax opinions on corporate reorganizations under I.R.C. {\S}368. To our knowledge, it is the first expert-annotated, tree-structured argument corpus for this domain. Explicit spans receive one of five functional labels: Rule, Analysis, Conclusion, Background Facts, and Procedural History. Rule, Analysis, and Conclusion spans can be linked into directed support trees, while Background Facts and Procedural History serve a contextual function. The corpus provides span-based, sentence-based, flat, and tree-structured representations. Agreement analysis shows that functional node labels are more reliable than directed support edges and implicit intermediate conclusions. Directed-path agreement is stronger than direct-edge agreement, which indicates that broad reachability is more stable than exact local decomposition. Classification experiments show that functional labels are learnable under case-disjoint evaluation. Retrieval experiments show that supervised fine-tuning improves within-case retrieval. However, cross-case generalization remains weak. The dataset supports legal passage classification and provides a conservative benchmark for structured argument mining in U.S. federal tax case law.

==> latex/figures_tables/query_representation.tex <==
\begin{figure}[t]
\centering

% -------------------- Main tree --------------------
\begin{forest}
tagtree
[{\texttt{[ARG]}}
  [{\texttt{[ROOT]}}
    [{\texttt{[CONCLUSION]}}]
  ]
  [{\texttt{[TREE]}}
    [{\texttt{[STEP]}}
      [{\texttt{[CONCL]}}
        [{\texttt{[ANALYSIS 2]}}]
      ]
      [{\texttt{[PREMISE]}}
        [{\texttt{[ANALYSIS 3]}}]
      ]
      [{\texttt{[PREMISE]}}
        [{\texttt{[MISSING]}}]
      ]
    ]
    [{\texttt{[STEP]}}
      [{\texttt{[CONCL]}}
        [{\texttt{[CONCLUSION]}}]
      ]
      [{\texttt{[PREMISE]}}
        [{\texttt{[ANALYSIS 2]}}]
      ]
      [{\texttt{[PREMISE]}}
        [{\texttt{[RULE 2]}}]
      ]
    ]
  ]
]
\end{forest}

\vspace{0.9em}

% -------------------- Focus --------------------
\begin{forest}
tagtree
[{\texttt{[FOCUS]}}
  [{\texttt{[STEP]}}
    [{\texttt{[CONCL]}}
      [{\texttt{[ANALYSIS 2]}}]
    ]
    [{\texttt{[PREMISE]}}
      [{\texttt{[ANALYSIS 3]}}]
    ]
    [{\texttt{[PREMISE]}}
      [{\texttt{[MASK]}}]
    ]
  ]
]
\end{forest}
\caption{Syllogistic argument tree and its linearized query representation.}
\label{fig:tree_retrieval_tag_map}
\end{figure}
